Foresight: Rapid Data Exploration Through Guideposts

Current tools for exploratory data analysis (EDA) require users to manually select data attributes, statistical computations and visual encodings. This can be daunting for large-scale, complex data. We introduce Foresight, a visualization recommender system that helps the user rapidly explore large high-dimensional datasets through "guideposts." A guidepost is a visualization corresponding to a pronounced instance of a statistical descriptor of the underlying data, such as a strong linear correlation between two attributes, high skewness or concentration about the mean of a single attribute, or a strong clustering of values. For each descriptor, Foresight initially presents visualizations of the "strongest" instances, based on an appropriate ranking metric. Given these initial guideposts, the user can then look at "nearby" guideposts by issuing "guidepost queries" containing constraints on metric type, metric strength, data attributes, and data values. Thus, the user can directly explore the network of guideposts, rather than the overwhelming space of data attributes and visual encodings. Foresight also provides for each descriptor a global visualization of ranking-metric values to both help orient the user and ensure a thorough exploration process. Foresight facilitates interactive exploration of large datasets using fast, approximate sketching to compute ranking metrics. We also contribute insights on EDA practices of data scientists, summarizing results from an interview study we conducted to inform the design of Foresight.

==> demo.tex <==
% !TEX root = paper.tex
% above command is for TeXShop

  We describe how an analyst uses \thetool to explore a dataset
  containing well-being indicators for the OECD member countries. This dataset
  contains 25 distinct attributes (indicators) for about 35 countries and is
  included in our demo mainly as an illustration and for ease of
  comprehension. \thetool is intended to facilitate interactive exploration
  of datasets with data items of the order of 100K having hundreds of attributes.

  The analyst loads the OECD dataset in Foresight and eyeballs
  various insights displayed in the carousels corresponding to
  each insight class (Figure~\ref{fig:teaser}).  She starts by checking univariate distributions as ranked by \thetool.  To gain
  intuition on  how the system ranks the histogram distributions, she flips
  back and forth the order of the rankings, and decides to keep the ranking
  criterion as she is happy what the system suggests. She notices that {\tt
  Personal Earnings} has the usual, skewed bimodal shape of an income
  distribution.  She can flip through the distributions carousel and
  bookmark (Figure~\ref{fig:foresightsidebar}) interesting insights to revisit later. In particular
  she bookmarks the {\tt Employees Working Very Long Hours} histogram, quickly
  checks the data points at the long tail of the distribution and takes note
  of the countries Turkey, Mexico, and Japan. The analyst wonders why Japan is
  there.

  She observes that a few data attributes have normal distributions but most have
  right or left skewed distributions.  She
  switches to the skewness criterion of \thetool ranking to focus on highly
  skewed attributes. \thetool suggests  {\tt Job Security } has the highest
  skew. Our analyst notes Turkey and Mexico are among the countries with lowest
  job security but surprisingly Japan is the country with highest job security.
  She next examines the outlier insights provided by \thetool.
  Enjoying the ease with which she can see which attributes have outliers, she saves
  the first three outlier insights, {\tt Homicide Rate}, {\tt Long Term
  Unemployment Rate}, and {\tt Education Attainment}. She also notes that Turkey and
  Mexico are outliers in {\tt Education Attainment}. Mexico is an outlier in
  {\tt Homicide Rate} but Turkey is not. Neither Turkey and nor Mexico seems
  to suffer, however, from a high {\tt Long Term Unemployment Rate}. Greece and Spain
  are outliers in this category.

  Already having a good sense of the data, our analyst moves
  to examine the correlations recommended by \thetool.
  She notes immediately that the indicators {\tt
  Working Long Hours} and {\tt Time Devoted To Leisure} have a strong negative
  correlation since this is one of the top ranked correlation insights
  recommended by Foresight. Encouraged with this quick discovery,
  she brings this insight \textit{into focus} and click on the related insights button.
  \thetool updates its recommendations by choosing a subset of insights within the neighborhood
  of the focused insight. The analyst explores the newly recommended correlations
  through multiple ranking metrics such as Pearson correlation coefficient,
   %and   Spearman rank correlation
  and is surprised to learn that {\tt Time Devoted To Leisure} has no correlation with {\tt Self Reported Health}.

  Intrigued with this lack of correlation, she checks the univariate
  distributional insight classes. The recommendations within these classes
  which have already been updated based the previous selections show that  {\tt
  Time Devoted To Leisure} has a Normal distribution while {\tt Self Reported
  Health} has a left-skewed distribution. Having gained greater familiarity
  with the OECD dataset, our analyst wonders about the factors that affect {\tt
  Self Reported Health}. She clicks on the distribution of \texttt{Self
  Reported Health} adding this as one of the focal insights. Foresight
  recommends a new set of correlated attributes in which she finds that {\tt
  Life Satisfaction} and {\tt Self Reported Health} are highly correlated.

  Satisfied with her preliminary discoveries (and armed with deeper questions
  about OECD countries than ever before), our analyst saves the current
  \thetool state to revisit later.


==> evaluation.tex <==
% !TEX root = paper.tex
% above command is for TeXShop
\subsection{User Study}
\input{userstudy}
\label{sec:userstudy}

\subsection{Performance Evaluation}
\input{performance}
\label{sec:performance}



==> interface.tex <==
% !TEX root = paper.tex
% above command is for TeXShop

%\begin{figure}[ht]
  %{\centering
  %\includegraphics[width=0.5\textwidth]{figures/foresightarch-sri}
  %\caption{Foresight Sketch \& Insight microservices are implemented as
  %RESTful R APIs. Foresight UI is implemented as an Angular-Meteor web app.\label{fig:foresightarch}}
  %}
%\end{figure}

Figure \ref{fig:foresightarch} presents the design of our prototype. The Foresight UI supports the
design criteria identified in Section \ref{sec:criteria} through the following
elements and controls.

\parhead{Guidepost Carousels:} Carousels are the primary mechanism by which guideposts are surfaced to the
user. Our prototype provides four carousels (see Figures \ref{fig:teaser} and \ref{fig:carousel}),
namely: a) distributions, corresponding to dispersion,
skewness, and heavy-tails descriptors, b) outliers, c) heterogenous frequencies, and d) correlations (linear relationships).
The three carousels corresponding to univariate insights are shown first followed by correlations.
Carousels provide controls for sorting the guideposts in ascending or descending order of the ranking metric. In addition,
descriptor-specific controls provide further options for visualization. For instance, by controlling the
number of histogram bins within the distribution carousel (Figures \ref{fig:teaser} and \ref{fig:carousel}),
the user can change the binning policy for histograms. Further, clicking on the overview button in
the correlations carousel (wheel icon in Figure \ref{fig:teaser}), the user can view the
overview visualization for linear relationships (Figure \ref{fig:corrheatmap}). Guidepost carousels support design
criteria 1, 2, 3, and 6.

\parhead{Data and Mode Control:} Foresight sidebar contains a file input element for users to
upload data (Figures \ref{fig:teaser} and \ref{fig:foresightsidebar}). As part of this initial interaction,
users can optionally specify if they wish to enable \textsc{sketch} mode for
insight computations or rely on \textsc{exact} mode. For data with number of numeric columns $\geq 500$, the default mode
is sketch, and the default is exact otherwise. This is in support of the $4^{th}$ design criterion.

\parhead{Expandable views and Bookmarks:} Hovering on a thumbnail within a carousel provides an expanded view
of the insight (Figure \ref{fig:carousel}), which the user can bookmark. Bookmarked insights are displayed on the
sidebar as part of \textsc{My Insights} section (Figure \ref{fig:foresightsidebar}).

\parhead{Related Insights:} Bookmarked insights in \textsc{My Insights} section contain
an action button for showing \textsc{related insights} (Figure \ref{fig:foresightsidebar}).
Clicking on this button will anchor a bookmarked insight, and filter the carousels thumbnails to the subset of insights that are
related to the anchored insight: specifically, an insight within a carousel is considered related if and only if it shares
at least one attribute (data column) with the anchored insight. This is in support of the $6^{th}$ criterion.

\parhead{Raw Data:} The input data is also displayed as a table and supports sorting and filtering across
columns as required by the $7^{th}$ criterion (Figure \ref{fig:teaser}).

%\begin{figure*}[t!]
%\centering
%\begin{minipage}[t]{0.218\textwidth}
  %\frame{\includegraphics[width=\linewidth]{figures/sidebarnav}}
  %\caption{UI Sidebar}
  %\label{fig:foresightsidebar}
%\end{minipage}\hfill
%\begin{minipage}[t]{0.76\textwidth}
  %\frame{\includegraphics[width=\linewidth]{figures/dispersion}}
  %\caption{Dispersion carousel which is part of the main panel in the Foresight UI}
  %\label{fig:carousel}
%\end{minipage}
%\end{figure*}
  %\begin{figure}[ht]
    %{\centering
    %\frame{\includegraphics[width=0.5\textwidth]{figures/corrplot_gray_labels}}
    %\caption{Overview visualization for correlations which is a heatmap of the correlation matrix
    %bi-clustered into groups of correlated columns.\label{fig:corrheatmap}}
    %}
  %\end{figure}


==> performance.tex <==
% !TEX root = paper.tex
% above command is for TeXShop

We conducted a variety of experiments with synthetic and real world datasets to gauge the performance of
exact correlation computation and sketching. The key performance metric of interest for exact computation is the response time.
For sketching, in addition to the response time, we are also interested in accuracy (Section \ref{sec:sketch}). We study
these metrics as a function of the data size (number of rows and columns) and the sketch cardinality, and discuss the regimes
where sketching significantly outperforms exact computation while maintaining high accuracy.
The correlation micro-service in the Foresight backend responds to a correlation query
in the form of a correlation matrix, where entry $(i, j)$ is the correlation coefficient between
columns $i$ and $j$ of the data matrix.
The response times reported in this section refer to the time elapsed between the correlation microservice
receiving a query and providing a response. We conducted all our experiments on commodity hardware with a
2.8 GHz Intel iCore CPU and 16 GB RAM.

\subsubsection{Datasets}
Our approach for generating synthetic data is based on other existing approaches for generating multi dimensional
correlated data~\cite{albuquerque:synthetic}. Given parameters $n$, $g$, and $r$ our data generator
creates a $n \times gr$ matrix whose columns are grouped in $g$ groups of $r$ columns each. Specifically,
for each column group $i$, we first generate a \textit{ground} column $\mathbf{g_j}$ of cardinality $n$,
whose entries are sampled independently from the Normal distribution $\mathcal{N}(0, \sigma_1^2)$.
In order to generate the $j^{th}$ column in this group, we create a \textit{perturbation} column $\mathbf{p_j}$
whose entries are sampled independently from the Normal distribution $\mathcal{N}(0, \sigma_2^2)$. The $j^{th}$
column in group $i$ is simply $\alpha_j \mathbf{g_i} + \mathbf{p_j}$, where the scaling factor $\alpha_j$
is sampled from $\mathcal{N}(0, 1)$. This scheme ensures that columns across groups are uncorrelated while
columns within group are positively or negatively correlated, with the extent of correlations dependent on the
ratio $\sigma_2 / \sigma_1$, and the scaling factor $\alpha_j$. In our experiments, we fixed $\sigma_1 = 5.0$ and $\sigma_2 = 1.0$, and we let
$n \in [1000, 2000, \ldots, 10000]$, $r = 100$, and $g \in [10, 20, \ldots, 70]$ yielding data matrices
whose size varied from $1000 \times 1000$ to $10000 \times 7000$.

In addition to the synthetic datasets, we experimented with three real world high-dimensional datasets from the
UCI machine learning repository~\cite{Lichman:2013}. These datasets belong to the following domains:
1) Arcene: cancer versus normal protein patterns
and their corresponding mass-spectrometric data of size $900 \times 10000$, 2) Mutants: p53 protein mutant data from
biophysical simulations of size $16772 \times 5409$, and 3) Gisette: handwriting and digit recognition dataset
of size $13500 \times 5000$.

Most figures presented in this subsection have best-fit curves superimposed
over data points: Figures \ref{fig:exactpredictor}, \ref{fig:totalsketchtime}, \ref{fig:sketchinittime},
\ref{fig:sketchtime}, and \ref{fig:exactsketchcompare} are
fitted with linear regression models, while Figures \ref{fig:quadraticexact} and \ref{fig:accuracy} are
fitted with \textit{loess} regression models~\cite{cleveland:loess}.


\subsubsection{Our Findings}
Figure \ref{fig:quadraticexact} presents the relationship between the response time of the
exact method as a function of the number of columns in the data. The response time for exact
computation is a \textit{quadratic function} of the number of columns. Figure \ref{fig:exactpredictor}
further confirms this showing a linear relationship between the response time of exact computation
and the product $nr^2$, where $n$ is the number of rows and $r$ is the number of numeric columns in the
data matrix. This is consistent with the fact that the exact computation of correlations involves
computation of the matrix product $\mathcal{Z}^{\top}{\mathcal{Z}}$, where $\mathcal{Z}$ is the mean subtracted
and normalized version of the matrix $\mathcal{B}$ consisting the $r$ numeric columns in the input dataset.

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{figures/quadraticexact}
\caption{Response time for exact computation is quadratically related to the number of columns.}
\label{fig:quadraticexact}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{figures/exactpredictor}
\caption{Response time for exact computation is linearly related to the product of data size and number of columns.}
\label{fig:exactpredictor}
\end{figure}

Figure \ref{fig:totalsketchtime} presents the response time for sketching as a function of data size for various sketch
cardinalities. While the response time of sketching appears to be linearly related to the data size as well as the
sketch cardinality, the goodness of fit for the various best-fit lines do not appear to be as
strong as that of Figure \ref{fig:exactpredictor}. To understand the factors affecting the response time of sketching
in greater depth, recall from section \ref{sec:sketch} that there are two phases in sketching, namely,
sketch initialization and sketch application. We instrumented our prototype to measure the runtimes of both
these phases individually; we present them in Figures \ref{fig:sketchinittime} and \ref{fig:sketchtime} respectively.

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{figures/totalsketchtime}
\caption{Response time for sketching vs data size for different sketch cardinality}
\label{fig:totalsketchtime}
\end{figure}

As Figure \ref{fig:sketchinittime} shows, sketch initialization time is a linear function of the product of data size and
sketch cardinality. This compares favourably with exact computation, whose response time is a
linear function of the product of data size and the number of columns. In other words, controlling for all other factors,
both the sketch initialization time and the response time for exact computation scale linearly as a function of data size;
however, the scaling factor for exact computation is the number of columns in the data while the scaling factor
for sketch initialization time is the sketch cardinality. A similar phenomenon is at play in terms of
the comparison between sketch application time and the response time of exact computation. As Figure \ref{fig:sketchtime}
shows, sketch application time is linearly related the product of sketch cardinality and the square of the number of columns.
Thus, controlling for all other factors, both the sketch application time, and the response time for exact computation
scale quadratically with the number of columns. However, the scaling factor for sketch application time is the sketch
cardinality while the scaling factor for the response time of exact computation is the number of rows in the data.
Since sketch cardinality is chosen to be significantly smaller than the number of rows or columns in
large high-dimensional datasets, one can expect significant savings in the total response time of sketching compared to
exact computation.

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{figures/sketchinittime}
\caption{Sketch initialization time is linearly related to the product of data size and sketch cardinality. Response time
for sketching $=$ sketch initialization time $+$ sketch runtime}
\label{fig:sketchinittime}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{figures/sketchtime}
\caption{Sketch runtime is linearly related to the product of sketch cardinality and the square of the number of columns. Response time
for sketching $=$ sketch initialization time $+$ sketch runtime}
\label{fig:sketchtime}
\end{figure}

The above hypothesis is confirmed by Figure \ref{fig:exactsketchcompare}. This figure compares response times for sketching and
exact computation. Clearly, response times for sketching is significantly better than exact computation at all cardinalities.
This is because sketch cardinality $\in [25, 50, \ldots, 250]$, while the number of rows and columns are respectively
$\in [1000, 2000, \ldots, 10000]$ and $\in [1000, 2000, \ldots, 7000]$ -- both significantly larger than
our maximum choice of sketch cardinality.

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{figures/exactsketchcompare}
\caption{Comparison of response times at number of columns $= 7000$. The top dashed line denotes the response time of exact
computation for various data sizes. The bottom most solid lines denote the response time of sketches of different cardinality
for various data sizes. Sketching significantly outperforms exact computation in terms of response time.
}
\label{fig:exactsketchcompare}
\end{figure}

Figure \ref{fig:accuracy} plots accuracy of sketching as a function of sketch cardinality.
A accuracy is a concave function of the sketch cardinality indicating that is a law of diminishing
returns at work in terms of the marginal utility gained through increased sketch cardinality. Further,
accuracy is primarily a function of sketch cardinality and largely independent of other factors such as
the number of rows or columns in the data. As can be seen from the figure, setting the sketch cardinality to $225$
or above typically ensures that the accuracy of sketching is above $90\%$.

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{figures/rmse}
\caption{Accuracy of sketching as a function of sketch cardinality for different data sizes. Accuracy
is largely independent of the data size and chiefly related to sketch cardinality. Sketch cardinality $\approx 225$ generally
suffices for ensuring accuracy $\approx 90\%$}
\label{fig:accuracy}
\end{figure}

Figure \ref{fig:realdata} presents our evaluation on three real world datasets.
We compare the response time of exact computation with sketch computation as well as the accuracy of sketching
at sketch cardinalities $200$ and $250$. The benefits of sketching as discussed in our evaluation with synthetic data
continue to hold with real datasets as well. Specifically, both the sketches achieve $> 90\%$ across
all datasets at a response time which is significantly smaller relative to exact computation.

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{figures/realdata}
\caption{Comparison of response times for exact computation and sketching for three real world high dimensional datasets. Sketching
significantly outperforms exact computation in terms of response times while achieving accuracy $\geq 90\%$}
\label{fig:realdata}
\end{figure}


==> userstudy.tex <==

To understand users' processes across two different approaches to exploratory analysis, we compare \thetool with Voyager 2, a recent visual
recommendation tool.  We hypothesized that \thetool would lead to a quicker
insight discovery and more hypothesis generation than Voyager 2 provides.
\noindent{\bf Participants: }
\noindent{\bf Tasks:} 
\\
T1: List unique hypothesis or insights that you find 

\noindent{\bf Protocol:}

\noindent{\bf Results:}

\noindent{\bf Discussion:}



